Lean-STaR: Learning to Interleave Thinking and Proving

Traditional language model-based theorem proving assumes that by training on a sufficient amount of formal proof data, a model will learn to prove theorems. Our key observation is that a wealth of informal information that is not present in formal proofs can be useful for learning to prove theorems. For instance, humans think through steps of a proof, but this thought process is not visible in the resulting code. We present Lean-STaR, a framework for training language models to produce informal thoughts prior to each step of a proof, thereby boosting the model's theorem-proving capabilities. Lean-STaR uses retrospective ground-truth tactics to generate synthetic thoughts for training the language model. At inference time, the trained model directly generates the thoughts prior to the prediction of the tactics in each proof step. Building on the self-taught reasoner framework, we then apply expert iteration to further fine-tune the model on the correct proofs it samples and verifies using the Lean solver. Lean-STaR achieves state-of-the-art results on the miniF2F-test benchmark within the Lean theorem proving environment, significantly outperforming base models ($\boldsymbol{43.4\% \rightarrow 46.3\%,}$ Pass@64). We also analyze the impact of the augmented thoughts on various aspects of the theorem proving process, providing insights into their effectiveness.

==> lstlean.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {
% Anything between $ becomes LaTeX math mode
mathescape=false,
% Comments may or not include Latex commands
texcl=false,

% keywords, list taken from lean-syntax.el
morekeywords=[1]{
import, prelude, protected, private, noncomputable, definition, meta, renaming,
hiding, parameter, parameters, begin, constant, constants,
lemma, variable, variables, theory,
print, theorem, example,
open, as, export, override, axiom, axioms, inductive, with,
structure, record, universe, universes,
alias, help, precedence, reserve, declare_trace, add_key_equivalence,
match, infix, infixl, infixr, notation, postfix, prefix, instance,
eval, reduce, check, end, this,
using, using_well_founded, namespace, section,
attribute, local, set_option, extends, include, omit, class,
raw, replacing,
calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
exists, if, dif, then, else, assume, obtain, from, register_simp_ext, unless, break, continue,
mutual, do, def, run_cmd, const,
partial, mut, where, macro, syntax, deriving,
return, try, catch, for, macro_rules, declare_syntax_cat, abbrev},

% Sorts
morekeywords=[2]{Sort, Type, Prop},

% tactics, list taken from lean-syntax.el
morekeywords=[3]{
assumption,
apply, intro, intros, allGoals,
generalize, clear, revert, done, exact,
refine, repeat, cases, rewrite, rw,
simp, simp_all, contradiction,
constructor, injection,
induction,
},

% modifiers, taken from lean-syntax.el
% note: 'otherkeywords' is needed because these use a different symbol.
% this command doesn't allow us to specify a number -- they are put with [1]
% otherkeywords={
% [persistent], [notation], [visible], [instance], [trans_instance],
% [class], [parsing-only], [coercion], [unfold_full], [constructor],
% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
% [whnf], [multiple_instances], [none], [decl], [declaration],
% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
% [localrefinfo], [recursor]
% },

% Various symbols
literate=
{α}{{\ensuremath{\mathrm{\alpha}}}}1
{β}{{\ensuremath{\mathrm{\beta}}}}1
{γ}{{\ensuremath{\mathrm{\gamma}}}}1
{δ}{{\ensuremath{\mathrm{\delta}}}}1
{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
{η}{{\ensuremath{\mathrm{\eta}}}}1
{θ}{{\ensuremath{\mathrm{\theta}}}}1
{ι}{{\ensuremath{\mathrm{\iota}}}}1
{κ}{{\ensuremath{\mathrm{\kappa}}}}1
{μ}{{\ensuremath{\mathrm{\mu}}}}1
{ν}{{\ensuremath{\mathrm{\nu}}}}1
{ξ}{{\ensuremath{\mathrm{\xi}}}}1
{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
{ρ}{{\ensuremath{\mathrm{\rho}}}}1
{σ}{{\ensuremath{\mathrm{\sigma}}}}1
{τ}{{\ensuremath{\mathrm{\tau}}}}1
{φ}{{\ensuremath{\mathrm{\varphi}}}}1
{χ}{{\ensuremath{\mathrm{\chi}}}}1
{ψ}{{\ensuremath{\mathrm{\psi}}}}1
{ω}{{\ensuremath{\mathrm{\omega}}}}1

{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
{Ω}{{\ensuremath{\mathrm{\Omega}}}}1

{ℵ}{{\ensuremath{\aleph}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1
{≠}{{\ensuremath{\neq}}}1
{≈}{{\ensuremath{\approx}}}1
{≡}{{\ensuremath{\equiv}}}1
{≃}{{\ensuremath{\simeq}}}1

{≤}{{\ensuremath{\leq}}}1
{≥}{{\ensuremath{\geq}}}1

{∂}{{\ensuremath{\partial}}}1
{∆}{{\ensuremath{\triangle}}}1 % or \laplace?

{∫}{{\ensuremath{\int}}}1
{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
{Π}{{\ensuremath{\mathrm{\Pi}}}}1

{⊥}{{\ensuremath{\perp}}}1
{∞}{{\ensuremath{\infty}}}1
{∂}{{\ensuremath{\partial}}}1

{∓}{{\ensuremath{\mp}}}1
{±}{{\ensuremath{\pm}}}1
{×}{{\ensuremath{\times}}}1

{⊕}{{\ensuremath{\oplus}}}1
{⊗}{{\ensuremath{\otimes}}}1
{⊞}{{\ensuremath{\boxplus}}}1

{∇}{{\ensuremath{\nabla}}}1
{√}{{\ensuremath{\sqrt}}}1

{⬝}{{\ensuremath{\cdot}}}1
{•}{{\ensuremath{\cdot}}}1
{∘}{{\ensuremath{\circ}}}1

%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
{⁻}{{\ensuremath{^{-}}}}1
{▸}{{\ensuremath{\blacktriangleright}}}1

{∧}{{\ensuremath{\wedge}}}1
{∨}{{\ensuremath{\vee}}}1
{¬}{{\ensuremath{\neg}}}1
{⊢}{{\ensuremath{\vdash}}}1

%{⟨}{{\ensuremath{\left\langle}}}1
%{⟩}{{\ensuremath{\right\rangle}}}1
{⟨}{{\ensuremath{\langle}}}1
{⟩}{{\ensuremath{\rangle}}}1

{↦}{{\ensuremath{\mapsto}}}1
{←}{{\ensuremath{\leftarrow}}}1
{<-}{{\ensuremath{\leftarrow}}}1
{→}{{\ensuremath{\rightarrow}}}1
{↔}{{\ensuremath{\leftrightarrow}}}1
{⇒}{{\ensuremath{\Rightarrow}}}1
{⟹}{{\ensuremath{\Longrightarrow}}}1
{⇐}{{\ensuremath{\Leftarrow}}}1
{⟸}{{\ensuremath{\Longleftarrow}}}1

{∩}{{\ensuremath{\cap}}}1
{∪}{{\ensuremath{\cup}}}1
{⊂}{{\ensuremath{\subseteq}}}1
{⊆}{{\ensuremath{\subseteq}}}1
{⊄}{{\ensuremath{\nsubseteq}}}1
{⊈}{{\ensuremath{\nsubseteq}}}1
{⊃}{{\ensuremath{\supseteq}}}1
{⊇}{{\ensuremath{\supseteq}}}1
{⊅}{{\ensuremath{\nsupseteq}}}1
{⊉}{{\ensuremath{\nsupseteq}}}1
{∈}{{\ensuremath{\in}}}1
{∉}{{\ensuremath{\notin}}}1
{∋}{{\ensuremath{\ni}}}1
{∌}{{\ensuremath{\notni}}}1
{∅}{{\ensuremath{\emptyset}}}1

{∖}{{\ensuremath{\setminus}}}1
{†}{{\ensuremath{\dag}}}1

{ℕ}{{\ensuremath{\mathbb{N}}}}1
{ℤ}{{\ensuremath{\mathbb{Z}}}}1
{ℝ}{{\ensuremath{\mathbb{R}}}}1
{ℚ}{{\ensuremath{\mathbb{Q}}}}1
{ℂ}{{\ensuremath{\mathbb{C}}}}1
{⌞}{{\ensuremath{\llcorner}}}1
{⌟}{{\ensuremath{\lrcorner}}}1
{⦃}{{\ensuremath{\{\!|}}}1
{⦄}{{\ensuremath{|\!\}}}}1

{‖}{{\ensuremath{\|}}}1
{₁}{{\ensuremath{_1}}}1
{₂}{{\ensuremath{_2}}}1
{₃}{{\ensuremath{_3}}}1
{₄}{{\ensuremath{_4}}}1
{₅}{{\ensuremath{_5}}}1
{₆}{{\ensuremath{_6}}}1
{₇}{{\ensuremath{_7}}}1
{₈}{{\ensuremath{_8}}}1
{₉}{{\ensuremath{_9}}}1
{₀}{{\ensuremath{_0}}}1
{ᵢ}{{\ensuremath{_i}}}1
{ⱼ}{{\ensuremath{_j}}}1
{ₐ}{{\ensuremath{_a}}}1

{¹}{{\ensuremath{^1}}}1

{ₙ}{{\ensuremath{_n}}}1
{ₘ}{{\ensuremath{_m}}}1
{ₚ}{{\ensuremath{_p}}}1
{↑}{{\ensuremath{\uparrow}}}1
{↓}{{\ensuremath{\downarrow}}}1

{...}{{\ensuremath{\ldots}}}1
{·}{{\ensuremath{\cdot}}}1

{▸}{{\ensuremath{\triangleright}}}1

{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
{\$}{{\color{symbolcolor}\$}}1

{:=}{{\color{symbolcolor}:=}}1
{=}{{\color{symbolcolor}=}}1
{<|>}{{\color{symbolcolor}<|>}}1
{<\$>}{{\color{symbolcolor}<\$>}}1
{+}{{\color{symbolcolor}+}}1
{*}{{\color{symbolcolor}*}}1,

% Comments
%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
morecomment=[s][\color{commentcolor}]{/-}{-/},
morecomment=[l][\itshape \color{commentcolor}]{--},

% Spaces are not displayed as a special character
showstringspaces=false,

% keep spaces
keepspaces=true,

% String delimiters
morestring=[b]",
morestring=[d],

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=false,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,
breakatwhitespace=true,

% Default style fors listingsred
basicstyle=\ttfamily\small,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,


% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the beginning of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{keywordcolor}},

% Style for sorts
keywordstyle=[2]{\ttfamily\color{sortcolor}},

% Style for tactics keywords
keywordstyle=[3]{\ttfamily\color{tacticcolor}},

% Style for attributes
keywordstyle=[4]{\ttfamily\color{attributecolor}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle={\ttfamily\footnotesize },

}



==> rebuttal.tex <==

\begin{figure*}[h!]
    \centering
    \begin{minipage}{0.32\textwidth}
    % \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/auto_figs/prm800k_7b_34b_min_prod-oprm_Level1-3.pdf}
    % \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
    % \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/auto_figs/prm800k_7b_34b_min_prod-oprm_Level4-5.pdf}
    % \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
    % \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/auto_figs/prm800k_7b_34b_min_prod-oprm_Level1-5.pdf}
    % \end{subfigure}
    \end{minipage}

    \begin{minipage}{0.32\textwidth}
    % \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/auto_figs/prm800k_34b_7b_min_prod-oprm_Level1-3.pdf}
    % \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
    % \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/auto_figs/prm800k_34b_7b_min_prod-oprm_Level4-5.pdf}
    % \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
    % \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/auto_figs/prm800k_34b_7b_min_prod-oprm_Level1-5.pdf}
    % \end{subfigure}
    \end{minipage}
    \caption{\red{Easy-to-hard generalization of evaluators applied to generators of different sizes. We evaluated 7b generator + 34b evaluator (upper) and 34b generator + 7b evaluator (lower). Both SFTs and RMs are trained on the easy data.}}
    \label{fig:easy-to-hard-evaluation-prm800k-cross-size}
    % \vspace{-10px}
\end{figure*}

\section{Revision: Main Results}

% \zs{Current Status of Available Results
% \\\\
% Here are the results ready to report in ICML submission (we need to generate more results to make the paper more solid before arXiving)
% \\\\
% On PRM800K (Done):\\
% \{7b\} x \{SFT, RM\} x \{Weighted MV, PPO\}
% \\\\
% On PRM800K\\
% (PPO TBD after ICML deadline):\\
% \{34b\} x \{SFT, RM\} x \{Weighted MV\}
% \\\\
% On MetaMath \& Math-Shepherd (Done):\\
% \{7b\} x \{SFT, RM\} x \{Weighted MV, PPO\}
% \\\\
% On MetaMath \& Math-Shepherd\\
% (All TBD after ICML deadline):\\
% \{34b\} x \{SFT, RM\} x \{Weighted MV, PPO?\}}


\begin{table*}[t]
\caption{
Comparing reinforcement learning (RL) approaches for easy-to-hard generalization. All methods are of 7b size and evaluated with greedy decoding.
\dag{} indicates the model is trained with additional final-answer labels on hard tasks (similar to \citet{singh2023beyond}), which is not strictly a easy-to-hard generalization setup.
}
\label{tab:rl_results}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccc}
\toprule
& \multirow{2}{*}{RL Data} & \multicolumn{2}{c}{Reward} & \multicolumn{3}{c}{Accuracy}\\
& & Final-Answer & Process RM & Easy (level 1-3) & Hard (level 4-5) & All \\
\midrule
\multicolumn{6}{l}{\it (SFT / PRM trained on level 1-3 of PRM800K)} \\
% \multirow{2}{*}{ReST} & Easy & Easy & Easy & - & - & \\
% \\
SFT &  &  & & 28.2 & 12.2 & 19.8 \\
ReST-EM & Easy & Easy & $\times$ & 33.2 & 12.6 & 22.4 \\
% ReST-EM & Easy & Easy & $\times$ & 34.9 & 8.4 & 21.0 \\
ReST-EM & Hard & Hard & $\times$ & 31.9 & 8.0 & 19.4 \\
ReST-EM\dag & All & All & $\times$ & 35.7 & 8.8 & 21.6 \\
% \midrule
Iterative DPO & Easy & Easy & $\surd$ & \underline{42.0} & 12.2 & 26.4\\
Iterative DPO\dag & All & All & $\surd$ & 38.2 & 11.5 & 24.2 \\
% \midrule
PPO & Easy & Easy & $\times$ & \underline{42.0} & \underline{14.1} & \underline{27.4} \\
PPO & Hard & Hard & $\times$ & 34.0 & 9.2 & 21.0 \\
PPO\dag & All & All & $\times$ & \underline{42.0} & 10.7 & 25.6 \\
PPO & All & Easy & $\surd$ & \textbf{45.4} & \textbf{14.9} & \textbf{29.4}\\
\midrule
\multicolumn{6}{l}{\it (SFT / PRM trained on level 1-5 of MetaMath / Math-Shepherd)} \\
\multicolumn{4}{l}{Llemma-based SFT SoTA (Ours)} & 51.7 & 13.7 & 31.4\\
\multicolumn{4}{l}{Previous RL SoTA \citep{wang2023math}} & - & - & 33.0\\
\midrule
\multicolumn{6}{l}{\it (SFT / PRM trained on level 1-3 of MetaMath / Math-Shepherd)} \\
SFT &  &  &  & 44.1 & 14.9 & 28.8\\
ReST-EM & Easy & Easy & $\times$ & 50.4 & 14.5 & 31.6\\
Iterative DPO & Easy & Easy & $\surd$ & \textbf{53.8} & \textbf{16.0} & \textbf{34.0}\\
\red{Iterative DPO} & \red{All} & \red{Easy} & \red{$\surd$} & \red{\underline{49.6}} & \red{10.7} & \red{29.2} \\
% \red{Iterative DPO} & \red{All} & \red{Easy} & \red{ORM} & \red{48.7} & \red{13.7} & \red{30.4} \\
Iterative DPO\dag & All & All & $\surd$ & 47.9 & 12.2 & 29.2\\
PPO & Easy & Easy & $\times$ & \underline{50.8} & \underline{15.3} & \underline{32.2} \\
PPO\dag & All & All & $\times$ & \underline{50.8} & 13.4 & 31.2 \\
PPO & All & Easy & $\surd$ & \textbf{53.8} & \textbf{16.0} & \textbf{34.0}\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\begin{table*}[h!]
\caption{
\red{Easy-to-hard generalization of evaluators on coding problems (APPS). Both SFTs and RMs are trained on the easy (Introductory) data. We found that outcome reward models trained on easy tasks can improve the re-ranking (Best-of-N) performance on hard (Interview \& Competition) coding problems.}
}
\label{tab:apps_results}
\vskip 0.1in
% \color{red}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{  
\begin{tabular}{lcccccccccccc}
\toprule
 & \multirow{1}{*}{SFT / ORM} & \multirow{2}{*}{Decoding} & \multicolumn{4}{c}{Average Accuracy (\%)} & \multicolumn{4}{c}{Strict Accuracy (\%)}\\
& \multirow{1}{*}{Train Data} & & Intro. & Inter. & Comp. & All & Intro. & Inter. & Comp. & All \\
\midrule
% \multicolumn{6}{l}{\it (SFT / PRM trained on level 1-3 of PRM800K)} \\
% \multicolumn{6}{l}{\it (SFT trained on APPS levels: Introductory, Interview \& Competition)} \\
\multirow{5}{*}{Code Llama - 7b} & All & Greedy & \textbf{31.4} & 15.5 & \textbf{12.2} & \textbf{18.0} & 17.0 & 2.3 & 2.0 & 5.2 \\
% \cmidrule{2-10}
% \multicolumn{6}{l}{\it (SFT / ORM trained on APPS levels: Introductory)} \\
& Easy & Greedy & 26.8 & 14.1 & 9.5 & 15.7 & 11.0 & 3.0 & 0.0 & 4.0 \\
& Easy & Best-of-$1$ & 25.4 & 12.0 & 0.1 & 13.5 & 16.0 & 2.7 & 0.0 & 4.8 \\
& Easy & Best-of-$4$ & 27.1 & 13.8 & 8.1 & 15.3 & 14.0 & 4.0 & 0.0 & 5.2 \\
& Easy & Best-of-$16$ & 29.7 & \textbf{16.3} & 11.3 & \textbf{18.0} & \textbf{19.0} & \textbf{5.0} & \textbf{3.0} & \textbf{7.4} \\
\midrule
\multirow{5}{*}{Code Llama - 34b} & All &Greedy & 37.6 & 19.9 & \textbf{11.3} & 21.7 & 22.0 & 5.0 & 2.0 & 7.8 \\
% \cmidrule{2-10}
& Easy &Greedy & 33.9 & 19.4 & 8.5 & 20.1 & 21.0 & 6.0 & 1.0 & 8.0 \\
& Easy &Best-of-$1$ & 28.5 & 14.5 & 4.4 & 15.3 & 21.0 & 3.3 & 0.0 & 6.2  \\
& Easy &Best-of-$4$ & 36.3 & 21.3 & 10.5 & 22.1 & 24.0 & 8.7 & 1.0 & 10.2 \\
& Easy &Best-of-$16$ & \textbf{45.9} & \textbf{25.8} & 10.0 & \textbf{26.6} & \textbf{30.0} & \textbf{10.7} & \textbf{3.0} & \textbf{13.0} \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}



\begin{table*}[h!]
\caption{
\red{Pass@N scores on coding problems (APPS). }
}
\label{tab:apps_pass_results}
\vskip 0.1in
% \color{red}
\begin{center}
\begin{small}
\begin{sc}
% \resizebox{\textwidth}{!}{  
\begin{tabular}{lcccccccc}
\toprule
 & \multirow{1}{*}{SFT / ORM} & \multirow{2}{*}{Decoding} & \multicolumn{4}{c}{Accuracy (\%)}\\
& \multirow{1}{*}{Train Data} & & Intro. & Inter. & Comp. & All \\
\midrule
% \multicolumn{6}{l}{\it (SFT / PRM trained on level 1-3 of PRM800K)} \\
% \multicolumn{6}{l}{\it (SFT trained on APPS levels: Introductory, Interview \& Competition)} \\
\multirow{3}{*}{Code Llama - 7b}
& Easy & Pass @ $1$ & 11.0 & 1.6 & 0.0 & 3.2 \\
& Easy & Pass @ $4$ & 20.0 & 4.7 & 2.0 & 7.2 \\
& Easy & Pass @ $16$ & 39.0 & 9.3 & 6.0 & 14.6 \\
\midrule
\multirow{3}{*}{Code Llama - 34b}
& Easy & Pass @ $1$ & 19.0 & 5.3 & 2.0 & 7.3 \\
& Easy & Pass @ $4$ & 32.0 & 10.7 & 3.0 & 13.4 \\
& Easy & Pass @ $16$ & 44.0 & 18.3 & 8.0 & 21.4 \\
\bottomrule
\end{tabular}
% }
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


% ...

\subsection{Easy-to-Hard Generalization of Evaluators}

The primary metric we use to assess the effectiveness of our process reward model is not the average accuracy of verifying each step in a solution but rather the overall performance achieved through re-ranking methods (See discussion in Sec.~\ref{sec:metrics}). We first use re-ranking to evaluate the easy-to-hard generalization performance of evaluators.

\begin{all_red}

\subsubsection{Re-ranking} \label{sec:re-ranking}

We consider two re-ranking strategies: Best-of-$n$ (or rejection sampling) and Weighted Voting.
In our easy-to-hard generalization setting, both SFT models and Reward Models (RMs) are trained on easier tasks (levels 1-3), but evaluated on all difficulty levels (1-5).
We compare the performance between majority voting (SFT only) and re-ranking (SFT + OPRM) on the PRM800K dataset in Figure \ref{fig:easy-to-hard-evaluation-prm800k}-\ref{fig:easy-to-hard-evaluation-prm800k-cross-size}, and the performance of different reward models (PRMs, ORMs, \& OPRMs) on the PRM800K dataset in Figure \ref{fig:compare-reward-models-7b}-\ref{fig:compare-reward-models-34b}.
Specifically, we use $\texttt{min}$ as the reward aggregation function for best-of-$n$ and $\texttt{prod}$ for weighted voting\footnote{See more detailed analysis of reward aggregation functions in Appendix.~\ref{app:reward-aggregation}.}.
The figures illustrate the performance of different decoding strategies or reward models under the same number of sampled solutions per problem. We have the following findings:

\paragraph{OPRMs outperforms ORMs and PRMs}
This confirms our hypothesis that Process Reward Models (PRMs) and Outcome Reward Models (ORMs) capture different aspects of task-solving processes. By integrating the strengths of both PRMs and ORMs, Outcome \& Process Reward Models (OPRMs) demonstrate superior performance. However, follow-up experiments conducted on the MetaMath/Math-Shepherd datasets do not demonstrate significant improvements from incorporating additional ORM training examples. This lack of enhancement may be attributed to the fact that Math-Shepherd is already generated from final-answer rewards. 
This suggests that there remains a substantial difference between process rewards labeled by humans (e.g., PRM800K) and those generated automatically (e.g., Math-Shepherd).

\end{all_red}

\paragraph{Weighted voting outshines Best-of-$n$}
This finding diverges from past research where minimal performance differences were observed between weighted voting and Best-of-$n$ \citep{lightman2023let,uesato2022solvingmath}.
Our hypothesis is that this discrepancy arises from our specific experiment, which involves training a less powerful base model (Llemma; \citealt{azerbayev2023llemma}) on more difficult tasks (MATH; \citealt{hendrycksmath2021}). This setup might diminish the effectiveness of the reward model, potentially leading to an over-optimization of rewards \citep{gao2023scaling}. Given these insights, weighted voting is preferred as the primary re-ranking method for further discussions. Nevertheless, Best-of-$n$ still achieves competitive performance to majority voting when producing only one full solution. In Figure~\ref{fig:easy-to-hard-evaluation-prm800k-cross-size}, we also find that the 34b evaluator can significantly improve the 7b generator, while the 7b evaluator can still improve the performance of the 34b generator.

\paragraph{Greater effectiveness of re-ranking on harder tasks:}
Weighted voting not only consistently surpasses majority voting but also shows a more pronounced advantage on harder tasks. This observation leads to the conclusion that \textit{evaluators demonstrate better easy-to-hard generalization capabilities in comparison to generators}. This motivates us to explore RL approaches that optimize the generator against the evaluator to further improve the performance of easy-to-hard generation.

% \paragraph{Scaling with SFT and RM Parameter Counts}
% It's noted that when SFT and RM are equally sized, Best-of-$n$ falls short compared to majority voting. Conversely, using a larger RM to select the best sample from a smaller SFT model brings Best-of-$n$’s performance up to par with majority voting. Nevertheless, weighted voting remains effective especially on hard tasks across different model scales.
% \end{itemize}

\subsubsection{Reinforcement Learning (RL)}

{Given the conclusion above, an important question arises: how can evaluators once again assist generators in achieving enhanced easy-to-hard generalization capabilities?} We further investigate the enhancement of policy models through RL, utilizing easy-to-hard evaluators as reward models.
Similar to re-ranking, SFT and PRM are only trained on easy data. For a fair comparison between PRM800K and MetaMath, we only use vanilla PRMs in the RL training. All the RL methods use the validation accuracy for selecting the best checkpoint\footnote{This includes stopping iterations in ReST-EM and iterative DPO, and stopping online steps in PPO.}.
Our comparison spans offline (ReST \& DPO) and online (PPO) RL algorithms under various training conditions:
% \begin{itemize}[leftmargin=*]

\textbf{Easy Questions \& Easy Final Answers:} The SFT model samples from easy questions and receives the corresponding Final-Answer and optional PRM rewards.

\textbf{All Questions \& Easy Final Answers:} This assumes access to a range of easy and hard problems for RL training, with rewards for hard tasks solely provided by the easy-to-hard evaluator.

\textbf{All Questions \& All Final Answers:} This setting uses all data with the corresponding final answers, which is similar to \citet{singh2023beyond}, but not strictly a easy-to-hard generalization setup.
% \end{itemize}

\begin{all_red}

Based on the results reported in Table~\ref{tab:rl_results}, we have the following findings:

\paragraph{DPO and PPO excel over ReST:} Among the RL algorithms trained on the PRM800K dataset, PPO emerges as the most effective, significantly surpassing both ReST and DPO. On the MetaMATH dataset, PPO and DPO achieve top performance, while ReST shows only marginal improvements over the SFT baseline.
The comparative analysis between DPO and PPO across the PRM800K and MetaMATH datasets indicates that while DPO's efficacy is on par with PPO given a high-quality SFT model as initialization, PPO's effectiveness is less contingent on the quality of the underlying SFT model \citep{ouyang2022training,rafailov2023direct}.

\paragraph{PRM rewards are more beneficial than Final-Answer rewards for hard tasks:} Notably, models trained with PRM rewards with human supervision on the easy tasks (achieving a top performance of 34.0) outperform the previous state-of-the-art model trained across all task levels (33.0). This highlights the effectiveness of leveraging easy-to-hard evaluations to improve generator performance across varying task difficulties.


\subsection{Easy-to-Hard Generalization on the Coding Domain}

We conduct further experiments in the coding domain with the APPS dataset \citep{hendrycks2021measuring}. Following \citet{lightman2023let}, we sub-sampled 500 questions from the original test set of APPS as our test set. Specifically, we sub-sampled 100 Introductory questions, 300 Interview questions, and 100 Competition questions, following the original distribution in the test set.

In Table~\ref{tab:apps_results}, we compare the performance of SFT-trained Code Llama \citep{roziere2023code} (7b \& 34b) with greedy decoding and best-of-N approach. In the latter, an Outcome Reward Model (ORM) of the same model size is trained to select the best coding one from N sampled solutions.

We found that while the reward model is only trained on the outcome supervision of easy (Introductory) data, it significantly improves the model performance on hard (Interview \& Competition) data. These findings extend the premise of easy-to-hard generalization beyond the confines of mathematical reasoning, suggesting its applicability across diverse domains.

\end{all_red}
